Complexity classifications for different equivalence and audit problems for Boolean circuits

We study Boolean circuits as a representation of Boolean functions and consider different equivalence, audit, and enumeration problems. For a number of restricted sets of gate types (bases) we obtain efficient algorithms, while for all other gate types we show these problems are at least NP-hard.

==> class02.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% 
% several hundred mathematical symbols



% large complexity classes
\newcommand\EXPSPACE{{\rm EXPSPACE}}
\newcommand\NEXPTIME{{\rm NEXPTIME}}
\newcommand\EXPTIME{{\rm EXPTIME}}
\newcommand\MIP{{\rm MIP}}
\newcommand\PH{{\rm PH}}
\newcommand\FPH{{\rm FPH}}
\newcommand\CH{{\rm CH}}
\newcommand\PP{{\rm PP}}
\newcommand\BPP{{\rm BPP}}
\newcommand\ZPP{{\rm ZPP}}
\newcommand\RP{{\rm RP}}
\renewcommand\P{{\rm P}}
\newcommand\FP{{\rm FP}}
\newcommand\NP{{\rm NP}}
\newcommand\BH{{\rm BH}}
\newcommand\UP{{\rm UP}}
\newcommand\US{{\rm US}}
\newcommand\oNP{{1\text{-}\NP}}
\newcommand\AM{{\rm AM}}
\newcommand\MA{{\rm MA}}
\newcommand\PSPACE{{\rm PSPACE}}
\newcommand\FPSPACE{{\rm FPSPACE}}
\newcommand\IP{{\rm IP}}
\newcommand\IPP{{\rm IPP}}
\newcommand\PCP{{\rm PCP}}
\newcommand\Sigp[1]{\Sigma^{\rm p}_{#1}}
\newcommand\Pip[1]{\Pi^{\rm p}_{#1}}
\newcommand\Deltap[1]{\Delta^{\rm p}_{#1}}
\newcommand\Thetap[1]{\Theta^{\rm p}_{#1}}
\newcommand\Sigpo[2]{\Sigma^{{\rm p},#2}_{#1}}
\newcommand\MidbitP{{\rm MidbitP}}
\newcommand\MODPH{\text{\rm MOD-PH}}
\newcommand\numP{{\rm\#P}}
\newcommand\GapP{{{\rm GapP}}}

% operators
\renewcommand\.{\mathop{\cdot}}
\newcommand\co{{{\rm co}}}
\newcommand\ex{\exists}
\newcommand\fall{\forall}
\let\cedille\c
\renewcommand\c{\mathord{\rm C}}
\newcommand\ceq{\c_=}
\newcommand\pari{\mathord{\oplus}}
\newcommand\num{\mathord{\rm\#}}
\newcommand\Mod{\mathord{\rm Mod}}
\newcommand\bpp{{\mbox{\rm BP}^{\rm p}}}
\newcommand\rp{{\mbox{\rm R}^{\rm p}}}


% small complexity classes
\newcommand\NC{{\rm NC}}
\renewcommand\L{{\rm L}}
\newcommand\FL{{\rm FL}}
\newcommand\LOGSPACE{{\rm LOGSPACE}}
\newcommand\NL{{\rm NL}}
\newcommand\FNC{{\rm FNC}}
\newcommand\AC{{\rm AC}}
\newcommand\DET{{\rm DET}}
\newcommand\SAC{{\rm SAC}}
\newcommand\FSAC{{\rm FSAC}}
\newcommand\SACe{{\rm SAC}^1}
\newcommand\NCe{{\rm NC}^1}
\newcommand\ACn{{\rm AC}^0}
\newcommand\FAC{{\rm FAC}}
\newcommand\ACCn{{\rm ACC}^0}
\newcommand\TC{{\rm TC}}
\newcommand\FTC{{\rm FTC}}
\newcommand\TCn{{\rm TC}^0}
\newcommand\BPNCe{{\rm BPNC}^1}
\newcommand\qNC{{\rm qNC}}
\newcommand\qNCe{{\rm qNC}^1}
\newcommand\qTCn{{\rm qTC}^0}
\newcommand\qACn{{\rm qAC}^0}
\newcommand\qACCn{{\rm qACC}^0}
\newcommand\DLT{{\rm DLT}}
\newcommand\DLOGTIME{{\rm DLOGTIME}}
\newcommand\NLOGTIME{{\rm NLOGTIME}}
\newcommand\FDLOGTIME{{\rm FDLOGTIME}}
\newcommand\ALOGTIME{{\rm ALOGTIME}}
\newcommand\LOGH{{\rm LOGH}}
\newcommand\DLINTIME{{\rm DLINTIME}}
\newcommand\DLIN{{\rm DLIN}}
\newcommand\NLIN{{\rm NLIN}}
\newcommand\LOGCFL{{\rm LOGCFL}}
\newcommand\POLYLOGTIME{{\rm POLYLOGTIME}}
\newcommand\FPOLYLOGTIME{{\rm FPOLYLOGTIME}}
\newcommand\POLYLOGSPACE{{\rm POLYLOGSPACE}}
\newcommand\PLT{\POLYLOGTIME}
\newcommand\PLS{\POLYLOGSPACE}
\newcommand\SC{{\rm SC}}
\newcommand\NSC{{\rm NSC}}



% logical classes
\newcommand\FO{\text{\rm FO}}

\newcommand\SO{{\rm SO}}
\newcommand\SOM{{\rm SOM}}


%optimization classes
\newcommand\PO{\text{\rm PO}}
\newcommand\NPO{\text{\rm NPO}}




% language classes
\newcommand\CSL{{\rm CSL}}
\newcommand\CFL{{\rm CFL}}
\newcommand\REG{{\rm REG}}
\newcommand\RE{{\rm r.e.}}


% problems
\newcommand\SAT{\text{\rm SAT}}
\newcommand\TSAT{\text{\rm 3SAT}}
\newcommand\CLIQUE{\text{\rm CLIQUE}}


% leaf languages
\newcommand\Leaf{{\rm Leaf}}
\newcommand\BLeaf{{\rm BLeaf}}
\newcommand\LeafP{\Leaf^\P}
\newcommand\BLeafP{\BLeaf^\P}
\newcommand\leafM{{\rm leafstring}^{M}}
\newcommand\LeafM{{\rm Leaf}^M}
\newcommand\leqplt{\leq^{{\rm plt}}_m}
\newcommand\LeafFA{\Leaf^{\text{\rm FA}}}

% reductions
\newcommand\leqlogm{\leq^{\rm log}_m}
\newcommand\eqlogm{\equiv^{\rm log}_m}
\newcommand\leqm{\leq^{\rm p}_m}
\newcommand\leqT{\leq^{\rm p}_{T}}
\newcommand\leqtt{\leq^p_{{tt}}}
\newcommand\leqbtt{\leq^p_{{btt}}}
\newcommand\leqctt{\leq^p_{{ctt}}}
%\newcommand{\leqo}{\mathord{\leq}}
\newcommand\leqo{{\mathcal{R}}}
\newcommand\leqcd{\leq_{{\rm cd}}}
\newcommand\leqproj{\leq_{{\it proj}}}
\newcommand\leqmet{\leq^{\rm p}_{{\it met}}}
\newcommand\eqcd{\equiv_{{\rm cd}}}
\newcommand\leqnc{\leq_{T}^{\NC}}
\newcommand\leqncet{\leq^{\NCe}_T}
\newcommand\leqnce{\leq^{\NCe}_m}
\newcommand\leqlog{\leq^{\log}_m}
\newcommand\leqlogT{\leq^{\log}_{1\text{\rm-T}}}
\newcommand\leqpeT{\leq^{\rm p}_{1\text{\rm-T}}}
\newcommand\leqr{\leq^{\CR}}

% measure and probability
%\newcommand\Mu[1]{\text{Prob}[#1]}
\newcommand\Mu[1]{\mu\left[#1\right]}
\newcommand\MuA[1]{\mu_A\left[#1\right]}
\newcommand\prob[1]{\text{\rm prob}\left[#1\right]}

% ressource bounds
\newcommand\poly{n^{O(1)}}
\newcommand\polylog{\log^{O(1)}n}
\newcommand\Poly{/{\rm Poly}}
\newcommand\pol{{\rm pol}}
\newcommand\Pol{{\rm Pol}}
\newcommand\const{{\rm const}}

% complexity measures
\newcommand\ntisp{\text{\rm NTIME-SPACE}}
\newcommand\dtisp{\text{\rm DTIME-SPACE}}
\newcommand\dtime{\text{\rm DTIME}}
\newcommand\fdtime{\text{\rm FDTIME}}
\newcommand\ntime{\text{\rm NTIME}}
\newcommand\dspace{\text{\rm DSPACE}}
\newcommand\fdspace{\text{\rm FDSPACE}}
\newcommand\nspace{\text{\rm NSPACE}}
\newcommand\atimespace{\text{\rm ATIME-SPACE}}
\newcommand\atime{\text{\rm ATIME}}
\newcommand\aspace{\text{\rm ASPACE}}
\newcommand\atisp{\text{\rm ATIME-SPACE}}
\newcommand\atial{\text{\rm ATIME-ALT}}
\newcommand\aalsp{\text{\rm AALT-SPACE}}
\newcommand\aspsi{\text{\rm ASPACE-TREESIZE}}
%
\newcommand\size{\text{\rm SIZE}}
\newcommand\depth{\text{\rm DEPTH}}
\newcommand\side{\text{\rm SIZE-DEPTH}}
\newcommand\usize{\text{\rm UnbSIZE}}
\newcommand\udepth{\text{\rm UnbDEPTH}}
\newcommand\uside{\text{\rm UnbSIZE-DEPTH}}
%
\newcommand\fsize{\text{\rm FSIZE}}
\newcommand\fdepth{\text{\rm FDEPTH}}
\newcommand\fside{\text{\rm FSIZE-DEPTH}}
\newcommand\fusize{\text{\rm FUnbSIZE}}
\newcommand\fudepth{\text{\rm FUnbDEPTH}}
\newcommand\fuside{\text{\rm FUnbSIZE-DEPTH}}

% calligraphics etc
\newcommand\CA{{\mathcal{A}}}
\newcommand\CC{{\mathcal{C}}}
\newcommand\CD{{\mathcal{D}}}
\newcommand\CP{{\mathcal{P}}}
\newcommand\CR{{\mathcal{R}}}
\newcommand\F{{\mathcal{F}}}
\newcommand\G{{\mathcal{G}}}
\newcommand\K{{\mathcal{K}}}
\newcommand\M{{\mathcal{M}}}
\newcommand\N{{\mathbb{N}}}	% for AMS
\renewcommand\O{{\mathcal{O}}}
\newcommand\R{{\mathcal{R}}}
\newcommand\Z{{\mathbb{Z}}}	% for AMS
\newcommand\Zz{\mathbb{Z}_2}	% for AMS

% useful gadgets
\newcommand\set[2]{\bigl\{\,#1\bigm| #2\,\bigr\}}
\newcommand\sset[1]{\{\,#1\,\}}
\newcommand\powerset[1]{\mathcal{P}(#1)}
\newcommand\pair[1]{\langle#1\rangle}
\newcommand\ceiling[1]{\lceil#1\rceil}
\newcommand\floor[1]{\lfloor#1\rfloor}
\newcommand\seq{\subseteq}
\newcommand\qes{\supseteq}
%\newcommand\implies{\Rightarrow}
% \newcommand\eqdef{=_{\rm def}}
\newcommand\eqdef{=} % Changed by Henning to remove "def" subscripts everywhere
% \newcommand\defeq{\,{}_{\rm def}\!\!=}
\newcommand\defeq{}% Changed by Henning to remove "def" subscripts everywhere
% \newcommand\iffdef{\Longleftrightarrow_{\rm def}}
\newcommand\iffdef{\Longleftrightarrow} % Changed by Henning to remove "def" subscripts everywhere
\newcommand\cond[1]{[\![#1]\!]}
\newcommand\quark{\kern.5em}
\newcommand\mathcalli[1]{\mathcal{#1}}	% for AMS-TeX
%\newcommand\mathcalli[1]{{\cal #1}}	% for non-AMS-TeX
%\newcommand\text[1]{\mbox{#1}}		% for non-AMS-TeX

% other useful symbols
\newcommand\B{\{0,1\}}
\newcommand\Bs{\{0,1\}^*}
\newcommand\Bp{\{0,1\}^+}
\newcommand\into{\rightarrow}
\newcommand\sLR{($\seq$): }
\newcommand\sRL{($\supseteq$): }
\newcommand\LR{($\Rightarrow$): }
\newcommand\RL{($\Leftarrow$): }
\newcommand\emptystring{\epsilon}
\newcommand\symdiff{\mathop{\Delta}}


==> macros02.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
% Sectioning
%



\def\labelitemi{--}


% sections:
%

\makeatletter
\renewcommand{\section}{\@startsection
    {section}%
    {1}%
    {0mm}%
    {-2\baselineskip}%
    {\baselineskip}%
    {\normalfont\large\bf}}
\renewcommand{\subsection}{\@startsection
    {subsection}%
    {1}%
    {0mm}%
    {-\baselineskip}%
    {.8\baselineskip}%
    {\normalfont\normalsize\bf}}
\makeatother



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
% Theorem environments and the like

% diverse layout changes
\makeatletter
\def\@begintheorem#1#2{\parskip0pt plus3pt\it \trivlist \item[\hskip
\labelsep{\bf #1\ #2.}]}
\def\@opargbegintheorem#1#2#3{\parskip0pt plus3pt\it \trivlist
      \item[\hskip \labelsep{\bf #1\ #2\ #3.}]}
\makeatother


% Environments with Text in Roman
% i.e.: Definitions

\makeatletter

\def\newdefinition#1{\@ifnextchar[{\@odefi{#1}}{\@ndefi{#1}}}

\def\@ndefi#1#2{%
\@ifnextchar[{\@xndefi{#1}{#2}}{\@yndefi{#1}{#2}}}

\def\@xndefi#1#2[#3]{\expandafter\@ifdefinable\csname #1\endcsname
{\@definecounter{#1}\@addtoreset{#1}{#3}%
\expandafter\xdef\csname the#1\endcsname{\expandafter\noexpand
  \csname the#3\endcsname \@deficountersep \@deficounter{#1}}%
\global\@namedef{#1}{\@defi{#1}{#2}}\global\@namedef{end#1}{\@enddefi}}}

\def\@yndefi#1#2{\expandafter\@ifdefinable\csname #1\endcsname
{\@definecounter{#1}%
\expandafter\xdef\csname the#1\endcsname{\@deficounter{#1}}%
\global\@namedef{#1}{\@defi{#1}{#2}}\global\@namedef{end#1}{\@enddefi}}}

\def\@odefi#1[#2]#3{\expandafter\@ifdefinable\csname #1\endcsname
  {\global\@namedef{the#1}{\@nameuse{the#2}}%
\global\@namedef{#1}{\@defi{#2}{#3}}%
\global\@namedef{end#1}{\@enddefi}}}

\def\@defi#1#2{\refstepcounter
    {#1}\@ifnextchar[{\@ydefi{#1}{#2}}{\@xdefi{#1}{#2}}}

\def\@xdefi#1#2{\@begindefi{#2}{\csname the#1\endcsname}\ignorespaces}
\def\@ydefi#1#2[#3]{\@opargbegindefi{#2}{\csname
       the#1\endcsname}{#3}\ignorespaces}

\def\@deficounter#1{\noexpand\arabic{#1}}
\def\@deficountersep{.}
%deleted September 2, 1986 MDK
%\def\@makethmnumber#1#2{\bf #1 #2:}
\def\@begindefi#1#2{\it \trivlist \item[\hskip \labelsep{\bf #1\ #2.}]\rm}
\def\@opargbegindefi#1#2#3{\it \trivlist
      \item[\hskip \labelsep{\bf #1\ #2\ #3.}]\rm}
\def\@enddefi{\endtrivlist}

\makeatother


%
% Environment-Vereinbarungen:

%\newtheorem{theorem}{Theorem}[section]
%\newtheorem{corollary}[theorem]{Corollary}
%\newtheorem{lemma}[theorem]{Lemma}
%\newtheorem{proposition}[theorem]{Proposition}
%\newtheorem{question}{Open Question}

%\newdefinition{definition}[theorem]{Definition}
%\newdefinition{example}[theorem]{Example}
%\newdefinition{problem}[theorem]{Problem}
%\newdefinition{remark}[theorem]{Remark}
%\newdefinition{observation}[theorem]{Observation}

% proof environment
%\newcommand\qedsymbol{\ding{113}}
\newcommand\qedsymbol{$\Box$}
\def\endproof{{\unskip\nobreak\hfil\penalty50
              \hskip1em\hbox{}\nobreak\qedsymbol
              \parfillskip=0pt\par\endtrivlist\addpenalty{-100}}}
\def\proof{\trivlist
    \penum=1%penum: siehe unten!
    \item[\hskip \labelsep{\it Proof.}]}

\def\endoutline{{\unskip\nobreak\hfil\penalty50
              \hskip1em\hbox{}\nobreak\qedsymbol
              \parfillskip=0pt\par\endtrivlist\addpenalty{-100}}}
\def\outline{\trivlist
    \penum=1%penum: siehe unten!
    \item[\hskip \labelsep{\it Proof sketch.}]}


% eigenes enumerate fuer Beweise etc., um Platz zu sparen ...
\newcount\penum
\def\pitem{\ifnum\penum>1\par\fi\the\penum. \advance\penum by1}

\newenvironment{penumerate}
  {\par\medskip\penum=1}{\par\medskip}


% problem environment
\newlength\problemlength
\settowidth{\problemlength}{\sl Question: }
%
\newcommand\problemdef[3]{%
\begin{list}{}{\labelwidth\problemlength \labelsep.7em \rightmargin1.5em
\leftmargin\problemlength \advance\leftmargin by3em%2em
%\leftmargin - \labelwidth - labelsep ergibt den linken Abstand zum Textrand
\parsep0ex \itemsep.2ex plus.1ex}
\item[{\sl Problem:\hfill}] #1
\item[{\sl Input:  \hfill}] #2
\item[{\sl Output: \hfill}] #3
\end{list}
}
%
\newlength\dproblength
\settowidth{\dproblength}{\textsl{Question: }}
\newcommand\dproblem[3]{%
\begin{list}{}{\labelwidth\dproblength \labelsep.5em \rightmargin0em
\leftmargin\dproblength \advance\leftmargin by2.3em
\parsep0ex \itemsep.2ex plus.1ex}
\item[{\textsl{Problem:}  \hfill}] #1
\item[{\textsl{Instance:} \hfill}] #2
\item[{\textsl{Question:} \hfill}] #3
\end{list}
}

% numerierte Gleichungen, Bemerkungen, etc;
% nur mit Nummer, ohne "Satz", "Korollar", ...

\newenvironment{eqn}
   {\trivlist\refstepcounter{theorem}\item[\hskip \labelsep{\bf \thetheorem.}]}
   {\endtrivlist}

\newcounter{noheadsectionctr}[section]
\def\noheadsection{\addtocounter{noheadsectionctr}{1}
    \par\noindent{\bf\arabic{section}.\arabic{noheadsectionctr}. }}

\newcounter{parctr}
%\newenvironment{numberedpar}
%   {\trivlist\stepcounter{parctr}\item[\hskip \labelsep{\bf \theparctr.}]}
%   {\endtrivlist}
\newenvironment{numberedpar}
   {\smallskip\stepcounter{parctr}\par\noindent{\bf\theparctr.}}
   {\smallskip}




\newcommand\Todo[1]{\par{\sl #1}}
\newcommand\todo[1]{$\triangleright$ {\sl #1} $\triangleleft$}
\newcommand\marg[1]{\marginpar{\raggedright\footnotesize\sl #1}}



% ragged-Kommandos in Paragraphen in Tabellen
% siehe LaTeX-Companion, p. 108
\newcommand\PreserveBackslash[1]{\let\temp=\\#1\let\\=\temp}
\newcommand\tableraggedright{\PreserveBackslash\raggedright}
\newcommand\tableraggedleft{\PreserveBackslash\raggedleft}
\newcommand\tablecentering{\PreserveBackslash\centering}
\newcommand{\var}[1]{\ensuremath{\text{\upshape{Var}}}(#1)}
